Semantic Composition in Visually Grounded Language Models

What is sentence meaning and its ideal representation? Much of the expressive power of human language derives from semantic composition, the mind's ability to represent meaning hierarchically & relationally over constituents. At the same time, much sentential meaning is outside the text and requires grounding in sensory, motor, and experiential modalities to be adequately learned. Although large language models display considerable compositional ability, recent work shows that visually-grounded language models drastically fail to represent compositional structure. In this thesis, we explore whether & how models compose visually grounded semantics, and how we might improve their ability to do so. Specifically, we introduce 1) WinogroundVQA, a new compositional visual question answering benchmark, 2) Syntactic Neural Module Distillation, a measure of compositional ability in sentence embedding models, 3) Causal Tracing for Image Captioning Models to locate neural representations vital for vision-language composition, 4) Syntactic MeanPool to inject a compositional inductive bias into sentence embeddings, and 5) Cross-modal Attention Congruence Regularization, a self-supervised objective function for vision-language relation alignment. We close by discussing connections of our work to neuroscience, psycholinguistics, formal semantics, and philosophy.

==> Chapters/List_of_Abbreviations.tex <==
% L I S T   O F   S Y M B O L S
% -----------------------------
% To include a Nomenclature section


%\addcontentsline{toc}{chapter}{\textbf{List of Acronyms}}
%\cleardoublepage
%\phantomsection	


%\renewcommand{\nomname}{List of Acronyms}
%\renewcommand{\nomAname}{\textbf{\large Abbreviations}}
%\textbf{List of Acronyms}



\chapter*{List of Abbreviations}
%\addcontentsline{toc}{chapter}{List of Acronyms}
\begin{longtable}{cp{0.8\textwidth}}


AI      &Artificial Intelligence.\\

\end{longtable}


\renewcommand{\nomGname}{\textbf{\large Mathematical Symbols}}
%\textbf{List of Symbols}

\renewcommand{\nomXname}{\textbf{\large Superscripts}}
\renewcommand{\nomZname}{\textbf{\large Subscripts}}

%\printnomenclature
%\cleardoublepage
%\phantomsection % allows hyperref to link to the correct page
% \newpage

==> private/declarationpage.tex <==
% D E C L A R A T I O N   P A G E
% -------------------------------

\begin{center}\textbf{Author's Declaration}\end{center}

  \noindent
I hereby declare that I am the sole author of this thesis. This is a true copy of the thesis, including any required final revisions, as accepted by my examiners.

  \bigskip
  
  \noindent
I understand that my thesis may be made electronically available to the public.

\cleardoublepage
%\newpage


==> private/examiners.tex <==
\cleardoublepage % Ends the current page and causes all figures and tables that have so far appeared in the input to be printed.
% In a two-sided printing style, it also makes the next page a right-hand (odd-numbered) page, producing a blank page if necessary.

 
% E X A M I N I N G   C O M M I T T E E (Required for MSc. and Ph.D. theses only)
% Remove or comment out the lines below to remove this page
\begin{center}\textbf{Examining Committee Membership}\end{center}
  \noindent
The following served on the Examining Committee for this thesis. The decision of the Examining Committee is by majority vote.
  \bigskip
  
  \noindent
\begin{tabbing}
Internal-External Member: \=  \kill % using longest text to define tab length
External Examiner: \>  Name X! \\ 
\> Professor, Dept. of, University of \\
\end{tabbing} 
  \bigskip
  
  \noindent
\begin{tabbing}
Internal-External Member: \=  \kill % using longest text to define tab length
Supervisor(s): \> Name 1!\\
\> Professor, Dept. of ML, \\Mohamed bin Zayed University of Artificial Intelligence (MBZUAI) \\
\> Name 2! \\
\> Professor , Dept. of CV, \\Mohamed bin Zayed University of Artificial Intelligence (MBZUAI) \\
\end{tabbing}
  \bigskip
  
  \noindent
  \begin{tabbing}
Internal-External Member: \=  \kill % using longest text to define tab length
Internal Member: \> Name Y! \\
\> Professor, Dept. of , University of  \\
\end{tabbing}
  \bigskip
  
  \noindent
\begin{tabbing}
Internal-External Member: \=  \kill % using longest text to define tab length
Internal-External Member: \> Name Z! \\
\> Professor, Dept. of , University of  \\
\end{tabbing}
  \bigskip
  
  \noindent
\begin{tabbing}
Internal-External Member: \=  \kill % using longest text to define tab length
Other Member(s): \> Name R! \\
\> Professor, Dept. of , University of \\
\end{tabbing}

\cleardoublepage

==> private/list-of-symbols.tex <==
% L I S T   O F   S Y M B O L S
% -----------------------------
% To include a Nomenclature section
\addcontentsline{toc}{chapter}{\textbf{Nomenclature}}

\renewcommand{\nomname}{Nomenclature}
\renewcommand{\nomAname}{\textbf{\large Abbreviations}}
\renewcommand{\nomGname}{\textbf{\large Mathematical Symbols}}
\renewcommand{\nomXname}{\textbf{\large Superscripts}}
\renewcommand{\nomZname}{\textbf{\large Subscripts}}

\printnomenclature
\cleardoublepage
\phantomsection % allows hyperref to link to the correct page
% \newpage






%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../uottawa-thesis"
%%% End: 
